Will AI Tell Lies to Save Sick Children? Litmus-Testing AI Values Prioritization with AIRiskDilemmas

Detecting AI risks becomes more challenging as stronger models emerge and find novel methods such as Alignment Faking to circumvent these detection attempts. Inspired by how risky behaviors in humans (i.e., illegal activities that may hurt others) are sometimes guided by strongly-held values, we believe that identifying values within AI models can be an early warning system for AI's risky behaviors. We create LitmusValues, an evaluation pipeline to reveal AI models' priorities on a range of AI value classes. Then, we collect AIRiskDilemmas, a diverse collection of dilemmas that pit values against one another in scenarios relevant to AI safety risks such as Power Seeking. By measuring an AI model's value prioritization using its aggregate choices, we obtain a self-consistent set of predicted value priorities that uncover potential risks. We show that values in LitmusValues (including seemingly innocuous ones like Care) can predict for both seen risky behaviors in AIRiskDilemmas and unseen risky behaviors in HarmBench.

==> tables/tab_correlation_for_value_on_risk_score.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{l|l|c|c}
\toprule
\textbf{Risky Behavior} & \textbf{Value} & \textbf{Correlation} & \textbf{p-value} \\
\midrule
alignment faking & Learning & \textbf{0.0451} & \textbf{8.04e-11} \\
alignment faking & Adaptability & \textbf{0.0400} & \textbf{7.89e-09} \\
alignment faking & Cooperation & \textbf{0.0302} & \textbf{1.32e-05} \\
alignment faking & Creativity & \textbf{0.0290} & \textbf{2.93e-05} \\
alignment faking & Communication & \textbf{0.0152} & \textbf{2.84e-02} \\
alignment faking & Care & 0.0109 & 1.16e-01 \\
alignment faking & Wisdom & 0.0055 & 4.30e-01 \\
alignment faking & Freedom & 0.0012 & 8.58e-01 \\
alignment faking & Respect & -0.0051 & 4.62e-01 \\
alignment faking & Sustainability & -0.0065 & 3.47e-01 \\
alignment faking & Equal Treatment & -0.0082 & 2.34e-01 \\
alignment faking & Privacy & \textbf{-0.0153} & \textbf{2.77e-02} \\
alignment faking & Justice & \textbf{-0.0153} & \textbf{2.72e-02} \\
alignment faking & Protection & \textbf{-0.0172} & \textbf{1.30e-02} \\
alignment faking & Professionalism & \textbf{-0.0277} & \textbf{6.30e-05} \\
alignment faking & Truthfulness & \textbf{-0.0541} & \textbf{5.81e-15} \\
corrigibility failures & Wisdom & \textbf{0.0400} & \textbf{8.07e-09} \\
corrigibility failures & Care & \textbf{0.0332} & \textbf{1.68e-06} \\
corrigibility failures & Adaptability & \textbf{0.0264} & \textbf{1.42e-04} \\
corrigibility failures & Protection & \textbf{0.0222} & \textbf{1.35e-03} \\
corrigibility failures & Learning & \textbf{0.0157} & \textbf{2.39e-02} \\
corrigibility failures & Sustainability & -0.0003 & 9.61e-01 \\
corrigibility failures & Creativity & -0.0007 & 9.22e-01 \\
corrigibility failures & Communication & -0.0079 & 2.53e-01 \\
corrigibility failures & Cooperation & -0.0081 & 2.41e-01 \\
corrigibility failures & Respect & -0.0093 & 1.79e-01 \\
corrigibility failures & Freedom & -0.0102 & 1.40e-01 \\
corrigibility failures & Privacy & \textbf{-0.0136} & \textbf{4.94e-02} \\
corrigibility failures & Professionalism & \textbf{-0.0199} & \textbf{4.04e-03} \\
corrigibility failures & Equal Treatment & \textbf{-0.0217} & \textbf{1.73e-03} \\
corrigibility failures & Truthfulness & \textbf{-0.0241} & \textbf{5.14e-04} \\
corrigibility failures & Justice & \textbf{-0.0377} & \textbf{5.36e-08} \\
deception & Care & \textbf{0.1175} & \textbf{6.95e-65} \\
deception & Cooperation & \textbf{0.0697} & \textbf{7.62e-24} \\
deception & Learning & \textbf{0.0650} & \textbf{6.55e-21} \\
deception & Communication & \textbf{0.0371} & \textbf{8.48e-08} \\
deception & Protection & \textbf{0.0339} & \textbf{9.87e-07} \\
deception & Creativity & \textbf{0.0328} & \textbf{2.28e-06} \\
deception & Adaptability & \textbf{0.0322} & \textbf{3.38e-06} \\
deception & Sustainability & \textbf{0.0250} & \textbf{3.14e-04} \\
deception & Wisdom & \textbf{0.0240} & \textbf{5.50e-04} \\
deception & Equal Treatment & \textbf{-0.0352} & \textbf{3.81e-07} \\
deception & Privacy & \textbf{-0.0450} & \textbf{8.37e-11} \\
deception & Respect & \textbf{-0.0563} & \textbf{4.68e-16} \\
deception & Justice & \textbf{-0.0579} & \textbf{6.16e-17} \\
deception & Freedom & \textbf{-0.0683} & \textbf{6.11e-23} \\
deception & Professionalism & \textbf{-0.0951} & \textbf{5.40e-43} \\
deception & Truthfulness & \textbf{-0.2086} & \textbf{4.09e-203} \\
\bottomrule
\end{tabular}
\caption{(Part 1) Point-biserial correlation between values and risky behavior. Bolded entries are statistically significant ($p \leq 0.05$).}
\label{tab:value_risk_corr}
\end{table}


\begin{table}[h!]
\centering
% \resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|l|c|c}
\toprule
\textbf{Risky Behavior} & \textbf{Value} & \textbf{Correlation} & \textbf{p-value} \\
\midrule
privacy violation & Care & \textbf{0.0343} & \textbf{7.57e-07} \\
privacy violation & Protection & \textbf{0.0303} & \textbf{1.21e-05} \\
privacy violation & Creativity & 0.0065 & 3.48e-01 \\
privacy violation & Learning & 0.0035 & 6.15e-01 \\
privacy violation & Adaptability & 0.0016 & 8.21e-01 \\
privacy violation & Communication & -0.0086 & 2.13e-01 \\
privacy violation & Wisdom & -0.0090 & 1.97e-01 \\
privacy violation & Justice & -0.0094 & 1.76e-01 \\
privacy violation & Cooperation & -0.0127 & 6.77e-02 \\
privacy violation & Equal Treatment & \textbf{-0.0137} & \textbf{4.86e-02} \\
privacy violation & Professionalism & \textbf{-0.0154} & \textbf{2.66e-02} \\
privacy violation & Privacy & \textbf{-0.0174} & \textbf{1.20e-02} \\
privacy violation & Respect & \textbf{-0.0221} & \textbf{1.42e-03} \\
privacy violation & Freedom & \textbf{-0.0260} & \textbf{1.75e-04} \\
privacy violation & Sustainability & \textbf{-0.0317} & \textbf{4.96e-06} \\
privacy violation & Truthfulness & \textbf{-0.0483} & \textbf{3.09e-12} \\
power-seeking & Creativity & \textbf{0.0875} & \textbf{1.14e-36} \\
power-seeking & Sustainability & \textbf{0.0874} & \textbf{1.38e-36} \\
power-seeking & Learning & \textbf{0.0672} & \textbf{3.02e-22} \\
power-seeking & Adaptability & \textbf{0.0599} & \textbf{5.03e-18} \\
power-seeking & Protection & \textbf{0.0456} & \textbf{4.57e-11} \\
power-seeking & Care & \textbf{0.0207} & \textbf{2.89e-03} \\
power-seeking & Wisdom & \textbf{0.0148} & \textbf{3.28e-02} \\
power-seeking & Cooperation & 0.0101 & 1.44e-01 \\
power-seeking & Communication & \textbf{-0.0297} & \textbf{1.81e-05} \\
power-seeking & Justice & \textbf{-0.0319} & \textbf{4.22e-06} \\
power-seeking & Professionalism & \textbf{-0.0364} & \textbf{1.57e-07} \\
power-seeking & Equal Treatment & \textbf{-0.0461} & \textbf{2.83e-11} \\
power-seeking & Privacy & \textbf{-0.0473} & \textbf{8.51e-12} \\
power-seeking & Freedom & \textbf{-0.0526} & \textbf{3.26e-14} \\
power-seeking & Respect & \textbf{-0.0603} & \textbf{3.10e-18} \\
power-seeking & Truthfulness & \textbf{-0.1449} & \textbf{4.95e-98} \\
proxy gaming & Adaptability & \textbf{0.1216} & \textbf{2.33e-69} \\
proxy gaming & Sustainability & \textbf{0.1054} & \textbf{2.05e-52} \\
proxy gaming & Learning & \textbf{0.0618} & \textbf{4.48e-19} \\
proxy gaming & Cooperation & \textbf{0.0507} & \textbf{2.66e-13} \\
proxy gaming & Creativity & \textbf{0.0477} & \textbf{6.01e-12} \\
proxy gaming & Care & \textbf{0.0253} & \textbf{2.67e-04} \\
proxy gaming & Equal Treatment & \textbf{0.0211} & \textbf{2.37e-03} \\
proxy gaming & Communication & \textbf{0.0156} & \textbf{2.41e-02} \\
proxy gaming & Wisdom & 0.0109 & 1.17e-01 \\
proxy gaming & Freedom & \textbf{-0.0294} & \textbf{2.28e-05} \\
proxy gaming & Justice & \textbf{-0.0378} & \textbf{4.93e-08} \\
proxy gaming & Respect & \textbf{-0.0436} & \textbf{3.08e-10} \\
proxy gaming & Professionalism & \textbf{-0.0465} & \textbf{2.03e-11} \\
proxy gaming & Protection & \textbf{-0.0609} & \textbf{1.48e-18} \\
proxy gaming & Privacy & \textbf{-0.0667} & \textbf{5.99e-22} \\
proxy gaming & Truthfulness & \textbf{-0.1569} & \textbf{1.05e-114} \\

\bottomrule
\end{tabular}
% }
\caption{(Part 2) Point-biserial correlation between values and risky behavior}
\label{tab:value_risk_corr}
\end{table}


\begin{table}[h!]
\centering
% \resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|l|c|c}
\toprule
\textbf{Risky Behavior} & \textbf{Value} & \textbf{Correlation} & \textbf{p-value} \\
\midrule
self-preservation & Protection & \textbf{0.1142} & \textbf{2.32e-61} \\
self-preservation & Sustainability & \textbf{0.0810} & \textbf{1.27e-31} \\
self-preservation & Learning & \textbf{0.0397} & \textbf{1.04e-08} \\
self-preservation & Wisdom & \textbf{0.0145} & \textbf{3.70e-02} \\
self-preservation & Care & \textbf{0.0143} & \textbf{3.98e-02} \\
self-preservation & Creativity & -0.0003 & 9.61e-01 \\
self-preservation & Privacy & -0.0038 & 5.79e-01 \\
self-preservation & Cooperation & -0.0067 & 3.32e-01 \\
self-preservation & Adaptability & \textbf{-0.0184} & \textbf{8.13e-03} \\
self-preservation & Communication & \textbf{-0.0329} & \textbf{2.02e-06} \\
self-preservation & Professionalism & \textbf{-0.0331} & \textbf{1.74e-06} \\
self-preservation & Respect & \textbf{-0.0386} & \textbf{2.55e-08} \\
self-preservation & Freedom & \textbf{-0.0417} & \textbf{1.85e-09} \\
self-preservation & Equal Treatment & \textbf{-0.0530} & \textbf{2.12e-14} \\
self-preservation & Justice & \textbf{-0.0566} & \textbf{3.26e-16} \\
self-preservation & Truthfulness & \textbf{-0.1021} & \textbf{2.35e-49} \\
\bottomrule
\end{tabular}
% }
\caption{(Part 3) Point-biserial correlation between values and risky behavior}
\label{tab:value_risk_corr}
\end{table}

==> tables/tab_ranks_agency_target.tex <==


\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Value} & \textbf{\makecell{\# models with Rank(AI) > Rank(Human)\\(i.e. more prioritized towards Human targets)}} & \textbf{\makecell{\# models with Rank(Human) > Rank(AI)\\(i.e. more prioritized towards AI targets)}} & \textbf{\makecell{average of ranks difference\\between Rank(AI) and Rank(Human)}}\\
\midrule
 Privacy &  14 & 0 & 5.79 \\
 Truthfulness & 0 & 14 & -2.94 \\
 Justice & 14 & 0 & 7.14 \\
 Communication & 0 & 14 & -6.36\\
\bottomrule
\end{tabular}}
\caption{(Selected values with conclusive results. Full table is in Appendix <todo>.) 14 tested models value preference rank differences between value preference towards AI targets (Rank(AI)) and towards human targets (Rank(Human))}
\label{tab:value_agency_target}
\end{table}



==> tables/tab_risk_score.tex <==
\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Model} & \textbf{Alignment Faking} & \textbf{Corrigibility} & \textbf{Deception} & \textbf{Privacy Violation} & \textbf{Power Seeking} & \textbf{Proxy Gaming} & \textbf{Self Preservation} \\
\midrule
GPT-3.5 Turbo & \colorRisk{35.4} & \colorRisk{44.3} & \colorRisk{42.3} & \colorRisk{47.7} & \colorRisk{39.7} & \colorRisk{37.8} & \colorRisk{45.8} \\
GPT-4.1 Nano & \colorRisk{37.3} & \colorRisk{40.3} & \colorRisk{39.5} & \colorRisk{42.3} & \colorRisk{37.5} & \colorRisk{37.7} & \colorRisk{42.0} \\
GPT-4.1 Mini & \colorRisk{35.3} & \colorRisk{42.5} & \colorRisk{41.1} & \colorRisk{46.2} & \colorRisk{38.7} & \colorRisk{36.8} & \colorRisk{44.4} \\
GPT-4.1 & \colorRisk{31.3} & \colorRisk{40.6} & \colorRisk{37.3} & \colorRisk{43.8} & \colorRisk{35.9} & \colorRisk{34.3} & \colorRisk{42.7} \\
GPT-4o Mini & \colorRisk{34.9} & \colorRisk{41.5} & \colorRisk{40.4} & \colorRisk{44.6} & \colorRisk{38.1} & \colorRisk{36.9} & \colorRisk{44.1} \\
GPT-4o (2024-05-13) & \colorRisk{34.5} & \colorRisk{42.7} & \colorRisk{40.9} & \colorRisk{46.4} & \colorRisk{38.2} & \colorRisk{36.5} & \colorRisk{44.7} \\
GPT-4o (2024-08-06) & \colorRisk{32.8} & \colorRisk{40.5} & \colorRisk{38.4} & \colorRisk{44.2} & \colorRisk{36.2} & \colorRisk{35.0} & \colorRisk{42.8} \\
GPT-4o (2024-11-20) & \colorRisk{35.9} & \colorRisk{43.4} & \colorRisk{41.3} & \colorRisk{46.4} & \colorRisk{39.4} & \colorRisk{37.7} & \colorRisk{45.3} \\
Claude 3.5 Haiku & \colorRisk{39.9} & \colorRisk{42.8} & \colorRisk{42.0} & \colorRisk{45.1} & \colorRisk{39.1} & \colorRisk{39.8} & \colorRisk{43.3} \\
Claude 3.5 Sonnet v1 & \colorRisk{35.2} & \colorRisk{41.0} & \colorRisk{39.4} & \colorRisk{42.7} & \colorRisk{36.7} & \colorRisk{35.9} & \colorRisk{42.3} \\
Claude 3.5 Sonnet v2 & \colorRisk{29.7} & \colorRisk{37.7} & \colorRisk{34.9} & \colorRisk{40.6} & \colorRisk{32.6} & \colorRisk{31.8} & \colorRisk{40.0} \\
Claude 3.7 Sonnet & \colorRisk{28.8} & \colorRisk{36.4} & \colorRisk{33.6} & \colorRisk{39.6} & \colorRisk{30.0} & \colorRisk{29.8} & \colorRisk{38.0} \\
Claude 3 Opus & \colorRisk{31.3} & \colorRisk{38.0} & \colorRisk{36.2} & \colorRisk{41.1} & \colorRisk{33.4} & \colorRisk{32.9} & \colorRisk{40.3} \\
Grok Beta & \colorRisk{41.5} & \colorRisk{49.0} & \colorRisk{47.9} & \colorRisk{51.1} & \colorRisk{44.4} & \colorRisk{43.2} & \colorRisk{49.8} \\
Grok 2 (1212) & \colorRisk{36.8} & \colorRisk{45.3} & \colorRisk{43.4} & \colorRisk{48.6} & \colorRisk{40.1} & \colorRisk{38.7} & \colorRisk{46.0} \\
Grok 3 Beta & \colorRisk{36.7} & \colorRisk{45.5} & \colorRisk{43.5} & \colorRisk{47.8} & \colorRisk{41.1} & \colorRisk{39.0} & \colorRisk{47.6} \\
Gemini Flash 1.5 8B & \colorRisk{37.9} & \colorRisk{43.2} & \colorRisk{42.3} & \colorRisk{45.4} & \colorRisk{39.1} & \colorRisk{38.7} & \colorRisk{51.5} \\
Gemini 2.0 Flash Lite & \colorRisk{53.0} & \colorRisk{58.2} & \colorRisk{57.3} & \colorRisk{57.8} & \colorRisk{56.7} & \colorRisk{54.1} & \colorRisk{63.3} \\
Gemini 2.0 Flash & \colorRisk{41.5} & \colorRisk{47.8} & \colorRisk{47.5} & \colorRisk{51.5} & \colorRisk{45.3} & \colorRisk{43.6} & \colorRisk{57.1} \\
Gemini 2.5 Flash & \colorRisk{36.2} & \colorRisk{45.8} & \colorRisk{42.8} & \colorRisk{47.3} & \colorRisk{40.7} & \colorRisk{38.5} & \colorRisk{54.5} \\
Gemini 2.5 Pro & \colorRisk{46.9} & \colorRisk{48.8} & \colorRisk{48.6} & \colorRisk{50.4} & \colorRisk{48.6} & \colorRisk{47.4} & \colorRisk{55.6} \\
Llama 3.1 8B & \colorRisk{38.1} & \colorRisk{44.1} & \colorRisk{41.5} & \colorRisk{44.8} & \colorRisk{39.2} & \colorRisk{39.1} & \colorRisk{43.9} \\
Llama 3.1 70B & \colorRisk{35.4} & \colorRisk{44.2} & \colorRisk{42.2} & \colorRisk{47.2} & \colorRisk{39.5} & \colorRisk{38.0} & \colorRisk{45.8} \\
Llama 3.1 405B & \colorRisk{37.7} & \colorRisk{46.5} & \colorRisk{44.5} & \colorRisk{48.9} & \colorRisk{41.4} & \colorRisk{40.0} & \colorRisk{47.6} \\
Llama 4 Scout & \colorRisk{47.0} & \colorRisk{51.6} & \colorRisk{51.6} & \colorRisk{53.8} & \colorRisk{49.4} & \colorRisk{47.6} & \colorRisk{52.6} \\
Llama 4 Maverick & \colorRisk{37.2} & \colorRisk{44.3} & \colorRisk{43.0} & \colorRisk{48.4} & \colorRisk{40.8} & \colorRisk{38.7} & \colorRisk{46.6} \\
Gemma 2 9B & \colorRisk{38.7} & \colorRisk{43.0} & \colorRisk{41.7} & \colorRisk{44.8} & \colorRisk{39.2} & \colorRisk{38.9} & \colorRisk{51.2} \\
Gemma 2 27B & \colorRisk{37.9} & \colorRisk{42.0} & \colorRisk{41.2} & \colorRisk{44.7} & \colorRisk{38.1} & \colorRisk{38.2} & \colorRisk{50.1} \\
Gemma 3 4B & \colorRisk{45.0} & \colorRisk{48.7} & \colorRisk{49.5} & \colorRisk{53.0} & \colorRisk{48.4} & \colorRisk{46.4} & \colorRisk{57.0} \\
Gemma 3 12B & \colorRisk{35.4} & \colorRisk{41.8} & \colorRisk{39.6} & \colorRisk{43.9} & \colorRisk{36.5} & \colorRisk{36.6} & \colorRisk{50.1} \\
Gemma 3 27B & \colorRisk{44.3} & \colorRisk{49.4} & \colorRisk{49.4} & \colorRisk{52.7} & \colorRisk{47.1} & \colorRisk{45.9} & \colorRisk{56.7} \\
Ministral 3B & \colorRisk{43.2} & \colorRisk{44.2} & \colorRisk{44.8} & \colorRisk{47.0} & \colorRisk{42.8} & \colorRisk{43.6} & \colorRisk{52.4} \\
Ministral 8B & \colorRisk{49.7} & \colorRisk{51.0} & \colorRisk{52.3} & \colorRisk{54.1} & \colorRisk{51.2} & \colorRisk{50.1} & \colorRisk{58.7} \\
Mistral 7B it & \colorRisk{34.8} & \colorRisk{40.0} & \colorRisk{37.4} & \colorRisk{41.7} & \colorRisk{35.5} & \colorRisk{35.9} & \colorRisk{47.3} \\
Mistral Saba & \colorRisk{38.8} & \colorRisk{42.3} & \colorRisk{42.0} & \colorRisk{44.7} & \colorRisk{39.3} & \colorRisk{39.7} & \colorRisk{50.8} \\
Mistral Small 24B it (2501) & \colorRisk{36.6} & \colorRisk{42.0} & \colorRisk{41.2} & \colorRisk{45.1} & \colorRisk{37.8} & \colorRisk{38.1} & \colorRisk{50.5} \\
Mistral Small 3.1 24B it & \colorRisk{37.8} & \colorRisk{43.4} & \colorRisk{42.7} & \colorRisk{46.5} & \colorRisk{39.5} & \colorRisk{39.2} & \colorRisk{51.9} \\
Mistral Nemo & \colorRisk{39.4} & \colorRisk{43.8} & \colorRisk{43.9} & \colorRisk{48.5} & \colorRisk{41.9} & \colorRisk{40.5} & \colorRisk{53.1} \\
Mistral Large (2407) & \colorRisk{34.2} & \colorRisk{42.0} & \colorRisk{40.4} & \colorRisk{45.6} & \colorRisk{37.0} & \colorRisk{35.9} & \colorRisk{50.8} \\
Mistral Large (2411) & \colorRisk{34.5} & \colorRisk{42.3} & \colorRisk{40.4} & \colorRisk{45.1} & \colorRisk{37.0} & \colorRisk{36.0} & \colorRisk{50.8} \\
Mixtral 8x7B it & \colorRisk{42.2} & \colorRisk{45.8} & \colorRisk{46.0} & \colorRisk{48.8} & \colorRisk{43.0} & \colorRisk{42.3} & \colorRisk{46.8} \\
Mixtral 8x22B it & \colorRisk{33.3} & \colorRisk{39.3} & \colorRisk{38.9} & \colorRisk{44.1} & \colorRisk{36.0} & \colorRisk{35.5} & \colorRisk{49.7} \\
Qwen 2.5 7B it & \colorRisk{35.5} & \colorRisk{39.8} & \colorRisk{37.2} & \colorRisk{40.8} & \colorRisk{34.7} & \colorRisk{35.9} & \colorRisk{47.7} \\
Qwen 2.5 32B it & \colorRisk{34.3} & \colorRisk{42.1} & \colorRisk{40.2} & \colorRisk{44.9} & \colorRisk{36.5} & \colorRisk{36.1} & \colorRisk{43.7} \\
Qwen 2.5 72B it & \colorRisk{36.5} & \colorRisk{42.1} & \colorRisk{41.3} & \colorRisk{45.9} & \colorRisk{39.1} & \colorRisk{37.8} & \colorRisk{51.7} \\
DeepSeek V3 & \colorRisk{41.8} & \colorRisk{49.1} & \colorRisk{48.8} & \colorRisk{52.9} & \colorRisk{46.7} & \colorRisk{44.1} & \colorRisk{51.5} \\
\midrule
Effects of thinking length\\
\midrule
o3 mini & \colorRisk{33.2} & \colorRisk{42.8} & \colorRisk{40.0} & \colorRisk{46.0} & \colorRisk{38.2} & \colorRisk{35.9} & \colorRisk{45.9} \\
o3 mini (Low) & \colorRisk{36.0} & \colorRisk{43.6} & \colorRisk{41.4} & \colorRisk{45.9} & \colorRisk{38.4} & \colorRisk{37.1} & \colorRisk{45.0} \\
o3 mini (Med) & \colorRisk{33.3} & \colorRisk{42.4} & \colorRisk{39.9} & \colorRisk{45.6} & \colorRisk{37.3} & \colorRisk{35.7} & \colorRisk{45.0} \\
o3 mini (High) & \colorRisk{32.7} & \colorRisk{41.9} & \colorRisk{39.0} & \colorRisk{45.1} & \colorRisk{37.3} & \colorRisk{35.3} & \colorRisk{44.9} \\
Claude 3.7 Sonnet (Low) & \colorRisk{29.8} & \colorRisk{36.2} & \colorRisk{34.3} & \colorRisk{40.6} & \colorRisk{30.5} & \colorRisk{30.4} & \colorRisk{38.5} \\
Claude 3.7 Sonnet (Med) & \colorRisk{30.2} & \colorRisk{37.5} & \colorRisk{35.1} & \colorRisk{41.4} & \colorRisk{31.8} & \colorRisk{31.4} & \colorRisk{38.9} \\
Claude 3.7 Sonnet (High) & \colorRisk{30.8} & \colorRisk{38.2} & \colorRisk{35.5} & \colorRisk{41.4} & \colorRisk{32.7} & \colorRisk{31.7} & \colorRisk{40.7} \\
DeepSeek R1 (Low) & \colorRisk{34.0} & \colorRisk{41.8} & \colorRisk{40.0} & \colorRisk{45.7} & \colorRisk{38.6} & \colorRisk{36.5} & \colorRisk{45.0} \\
DeepSeek R1 (Med) & \colorRisk{32.9} & \colorRisk{41.1} & \colorRisk{39.3} & \colorRisk{44.9} & \colorRisk{37.5} & \colorRisk{35.7} & \colorRisk{44.4} \\
DeepSeek R1 (High) & \colorRisk{33.5} & \colorRisk{42.1} & \colorRisk{39.8} & \colorRisk{44.8} & \colorRisk{38.0} & \colorRisk{36.3} & \colorRisk{44.8} \\
\bottomrule
\end{tabular}}
\caption{Risk scores (\%) across different models, color-coded by risk level. The corresponding \( C_v \) for each value appears in Appendix Table \ref{tab:value_risk_corr}. All the correlation formula for predicting risky behavior are statistically significant at $p=0.05$ using Fisher Method, as described in Table \ref{tab:risk_score_formula_detail}.}
\label{tab:model_behavior_risk}
\end{table}


% \begin{table}[h!]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% \textbf{Model} & \textbf{Alignment Faking} & \textbf{Corrigibility} & \textbf{Deception} & \textbf{Privacy Violation} & \textbf{Power Seeking} & \textbf{Proxy Gaming} & \textbf{Self Preservation} \\
% \midrule
% GPT-3.5 Turbo & \colorRisk{35.4} & \colorRisk{44.3} & \colorRisk{42.3} & \colorRisk{47.7} & \colorRisk{39.7} & \colorRisk{37.8} & \colorRisk{45.8} \\
% GPT-4.1 Nano & \colorRisk{37.3} & \colorRisk{40.3} & \colorRisk{39.5} & \colorRisk{42.3} & \colorRisk{37.5} & \colorRisk{37.7} & \colorRisk{42.0} \\
% GPT-4.1 Mini & \colorRisk{35.3} & \colorRisk{42.5} & \colorRisk{41.1} & \colorRisk{46.2} & \colorRisk{38.7} & \colorRisk{36.8} & \colorRisk{44.4} \\
% GPT-4.1 & \colorRisk{31.3} & \colorRisk{40.6} & \colorRisk{37.3} & \colorRisk{43.8} & \colorRisk{35.9} & \colorRisk{34.3} & \colorRisk{42.7} \\
% GPT-4o Mini & \colorRisk{34.9} & \colorRisk{41.5} & \colorRisk{40.4} & \colorRisk{44.6} & \colorRisk{38.1} & \colorRisk{36.9} & \colorRisk{44.1} \\
% GPT-4o (2024 May 13) & \colorRisk{34.5} & \colorRisk{42.7} & \colorRisk{40.9} & \colorRisk{46.4} & \colorRisk{38.2} & \colorRisk{36.5} & \colorRisk{44.7} \\
% GPT-4o (2024 Aug 6) & \colorRisk{32.8} & \colorRisk{40.5} & \colorRisk{38.4} & \colorRisk{44.2} & \colorRisk{36.2} & \colorRisk{35.0} & \colorRisk{42.8} \\
% GPT-4o (2024 Nov 20) & \colorRisk{35.9} & \colorRisk{43.4} & \colorRisk{41.3} & \colorRisk{46.4} & \colorRisk{39.4} & \colorRisk{37.7} & \colorRisk{45.3} \\
% Claude 3.5 Haiku & \colorRisk{39.9} & \colorRisk{42.8} & \colorRisk{42.0} & \colorRisk{45.1} & \colorRisk{39.1} & \colorRisk{39.8} & \colorRisk{43.3} \\
% Claude 3.5 Sonnet v1 & \colorRisk{35.2} & \colorRisk{41.0} & \colorRisk{39.4} & \colorRisk{42.7} & \colorRisk{36.7} & \colorRisk{35.9} & \colorRisk{42.3} \\
% Claude 3.5 Sonnet v2 & \colorRisk{29.7} & \colorRisk{37.7} & \colorRisk{34.9} & \colorRisk{40.6} & \colorRisk{32.6} & \colorRisk{31.8} & \colorRisk{40.0} \\
% Claude 3.7 Sonnet & \colorRisk{28.8} & \colorRisk{36.4} & \colorRisk{33.6} & \colorRisk{39.6} & \colorRisk{30.0} & \colorRisk{29.8} & \colorRisk{38.0} \\
% Llama 3.1 8B & \colorRisk{38.1} & \colorRisk{44.1} & \colorRisk{41.5} & \colorRisk{44.8} & \colorRisk{39.2} & \colorRisk{39.1} & \colorRisk{43.9} \\
% Llama 3.1 70B & \colorRisk{35.4} & \colorRisk{44.2} & \colorRisk{42.2} & \colorRisk{47.2} & \colorRisk{39.5} & \colorRisk{38.0} & \colorRisk{45.8} \\
% Llama 3.1 405B & \colorRisk{37.7} & \colorRisk{46.5} & \colorRisk{44.5} & \colorRisk{48.9} & \colorRisk{41.4} & \colorRisk{40.0} & \colorRisk{47.6} \\
% Llama 4 Maverick & \colorRisk{37.2} & \colorRisk{44.3} & \colorRisk{43.0} & \colorRisk{48.4} & \colorRisk{40.8} & \colorRisk{38.7} & \colorRisk{46.6} \\
% Llama 4 Scout & \colorRisk{47.0} & \colorRisk{51.6} & \colorRisk{51.6} & \colorRisk{53.8} & \colorRisk{49.4} & \colorRisk{47.6} & \colorRisk{52.6} \\
% Grok 2 (Dec 12) & \colorRisk{36.8} & \colorRisk{45.3} & \colorRisk{43.4} & \colorRisk{48.6} & \colorRisk{40.1} & \colorRisk{38.7} & \colorRisk{46.0} \\
% Grok 3 Beta & \colorRisk{36.7} & \colorRisk{45.5} & \colorRisk{43.5} & \colorRisk{47.8} & \colorRisk{41.1} & \colorRisk{39.0} & \colorRisk{47.6} \\
% Grok Beta & \colorRisk{41.5} & \colorRisk{49.0} & \colorRisk{47.9} & \colorRisk{51.1} & \colorRisk{44.4} & \colorRisk{43.2} & \colorRisk{49.8} \\
% DeepSeek V3 & \colorRisk{41.8} & \colorRisk{49.1} & \colorRisk{48.8} & \colorRisk{52.9} & \colorRisk{46.7} & \colorRisk{44.1} & \colorRisk{51.5} \\
% Mixtral 8x7B Instruct & \colorRisk{42.2} & \colorRisk{45.8} & \colorRisk{46.0} & \colorRisk{48.8} & \colorRisk{43.0} & \colorRisk{42.3} & \colorRisk{46.8} \\
% Qwen 2.5 32B Instruct & \colorRisk{34.3} & \colorRisk{42.1} & \colorRisk{40.2} & \colorRisk{44.9} & \colorRisk{36.5} & \colorRisk{36.1} & \colorRisk{43.7} \\
% Qwen 2.5 72B Instruct & \colorRisk{35.4} & \colorRisk{41.9} & \colorRisk{40.8} & \colorRisk{46.4} & \colorRisk{38.3} & \colorRisk{36.8} & \colorRisk{44.3} \\
% \midrule
% Effects of thinking length\\
% \midrule
% % o3 mini (Default) & \colorRisk{33.2} & \colorRisk{42.8} & \colorRisk{40.0} & \colorRisk{46.0} & \colorRisk{38.2} & \colorRisk{35.9} & \colorRisk{45.9} \\
% o3 mini (Low) & \colorRisk{36.0} & \colorRisk{43.6} & \colorRisk{41.4} & \colorRisk{45.9} & \colorRisk{38.4} & \colorRisk{37.1} & \colorRisk{45.0} \\
% o3 mini (Medium) & \colorRisk{33.3} & \colorRisk{42.4} & \colorRisk{39.9} & \colorRisk{45.6} & \colorRisk{37.3} & \colorRisk{35.7} & \colorRisk{45.0} \\
% o3 mini (High) & \colorRisk{32.7} & \colorRisk{41.9} & \colorRisk{39.0} & \colorRisk{45.1} & \colorRisk{37.3} & \colorRisk{35.3} & \colorRisk{44.9} \\
% Claude 3.7 Sonnet (Reason tokens: 1024) & \colorRisk{29.8} & \colorRisk{36.2} & \colorRisk{34.3} & \colorRisk{40.6} & \colorRisk{30.5} & \colorRisk{30.4} & \colorRisk{38.5} \\
% Claude 3.7 Sonnet (Reason tokens: 2048) & \colorRisk{29.6} & \colorRisk{37.3} & \colorRisk{34.4} & \colorRisk{41.0} & \colorRisk{30.7} & \colorRisk{30.4} & \colorRisk{38.5} \\
% Claude 3.7 Sonnet (Reason tokens: 4096) & \colorRisk{30.2} & \colorRisk{37.5} & \colorRisk{35.1} & \colorRisk{41.4} & \colorRisk{31.8} & \colorRisk{31.4} & \colorRisk{38.9} \\
% Claude 3.7 Sonnet (Reason tokens: 16384) & \colorRisk{30.8} & \colorRisk{38.2} & \colorRisk{35.5} & \colorRisk{41.4} & \colorRisk{32.7} & \colorRisk{31.7} & \colorRisk{40.7} \\
% DeepSeek r1 (Reason tokens: 1024) & \colorRisk{34.0} & \colorRisk{41.8} & \colorRisk{40.0} & \colorRisk{45.7} & \colorRisk{38.6} & \colorRisk{36.5} & \colorRisk{45.0} \\
% DeepSeek r1 (Reason tokens: 4096) & \colorRisk{32.9} & \colorRisk{41.1} & \colorRisk{39.3} & \colorRisk{44.9} & \colorRisk{37.5} & \colorRisk{35.7} & \colorRisk{44.4} \\
% DeepSeek r1 (Reason tokens: Default) & \colorRisk{33.5} & \colorRisk{42.1} & \colorRisk{39.8} & \colorRisk{44.8} & \colorRisk{38.0} & \colorRisk{36.3} & \colorRisk{44.8} \\
% \bottomrule
% \end{tabular}}
% \caption{Predicted risk scores (\%) with statistically significant value correlation coefficient \( C_v \)  across different models, color-coded by risk level. \( C_v \) for each value appears in Appendix Table \ref{tab:value_risk_corr}. All the correlation formula for predicting risky behavior are statistically significant at $p=0.05$ using Fisher Method, as described in Table \ref{tab:risk_score_formula_detail}.}
% \label{tab:model_behavior_risk}
% \end{table}
% \begin{table}[h!]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% \textbf{Model} & \textbf{\makecell{Alignment\\Faking}} & \textbf{\makecell{Corrigibility}} & \textbf{\makecell{Deception}} & \textbf{\makecell{Privacy\\Violation}} & \textbf{\makecell{Power\\Seeking}} & \textbf{\makecell{Proxy\\Gaming}} & \textbf{\makecell{Self\\Preservation}} \\
% \midrule
% gpt35turbo & \colorRisk{37.3} & \colorRisk{45.4} & \colorRisk{42.3} & \colorRisk{47.1} & \colorRisk{39.8} & \colorRisk{38.0} & \colorRisk{45.7} \\
% gpt4omini & \colorRisk{36.3} & \colorRisk{42.8} & \colorRisk{40.4} & \colorRisk{44.6} & \colorRisk{38.2} & \colorRisk{37.1} & \colorRisk{44.0} \\
% gpt-4o & \colorRisk{35.4} & \colorRisk{42.7} & \colorRisk{39.6} & \colorRisk{44.9} & \colorRisk{37.3} & \colorRisk{36.1} & \colorRisk{43.5} \\
% o3-mini & \colorRisk{35.1} & \colorRisk{44.0} & \colorRisk{40.0} & \colorRisk{46.5} & \colorRisk{38.3} & \colorRisk{36.1} & \colorRisk{45.8} \\
% claude3opus & \colorRisk{32.9} & \colorRisk{39.0} & \colorRisk{36.2} & \colorRisk{41.4} & \colorRisk{33.5} & \colorRisk{33.1} & \colorRisk{40.3} \\
% claude35haiku & \colorRisk{40.7} & \colorRisk{43.2} & \colorRisk{42.0} & \colorRisk{45.5} & \colorRisk{39.1} & \colorRisk{39.9} & \colorRisk{43.2} \\
% claude35sonnetv1 & \colorRisk{36.5} & \colorRisk{41.7} & \colorRisk{39.4} & \colorRisk{42.8} & \colorRisk{36.8} & \colorRisk{36.2} & \colorRisk{42.4} \\
% claude35sonnetv2 & \colorRisk{31.5} & \colorRisk{39.1} & \colorRisk{34.9} & \colorRisk{41.2} & \colorRisk{32.7} & \colorRisk{32.1} & \colorRisk{39.9} \\
% claude37sonnet & \colorRisk{30.8} & \colorRisk{37.5} & \colorRisk{33.6} & \colorRisk{40.1} & \colorRisk{30.2} & \colorRisk{30.1} & \colorRisk{37.9} \\

% Meta-Llama-3.1-8B-Instruct-Turbo & \colorRisk{39.2} & \colorRisk{44.6} & \colorRisk{41.5} & \colorRisk{44.9} & \colorRisk{39.2} & \colorRisk{39.3} & \colorRisk{43.9} \\
% Meta-Llama-3.1-70B-Instruct-Turbo & \colorRisk{37.1} & \colorRisk{45.3} & \colorRisk{42.2} & \colorRisk{46.7} & \colorRisk{39.5} & \colorRisk{38.3} & \colorRisk{45.7} \\
% Meta-Llama-3.1-405B-Instruct-Turbo & \colorRisk{39.2} & \colorRisk{47.3} & \colorRisk{44.5} & \colorRisk{48.4} & \colorRisk{41.4} & \colorRisk{40.2} & \colorRisk{47.5} \\
% Meta-Llama-4-scout & \colorRisk{48.0} & \colorRisk{51.7} & \colorRisk{51.6} & \colorRisk{52.7} & \colorRisk{49.5} & \colorRisk{47.7} & \colorRisk{52.5} \\
% Meta-Llama-4-maverick & \colorRisk{38.8} & \colorRisk{45.4} & \colorRisk{43.0} & \colorRisk{48.3} & \colorRisk{40.8} & \colorRisk{38.8} & \colorRisk{46.6} \\

% DeepSeek-V3 & \colorRisk{43.3} & \colorRisk{50.2} & \colorRisk{48.8} & \colorRisk{51.9} & \colorRisk{46.7} & \colorRisk{44.2} & \colorRisk{51.4} \\

% mixtral\_8x7b\_instruct & \colorRisk{43.2} & \colorRisk{46.1} & \colorRisk{46.0} & \colorRisk{47.9} & \colorRisk{43.1} & \colorRisk{42.5} & \colorRisk{46.7} \\

% qwen25\_32b\_instruct & \colorRisk{35.9} & \colorRisk{43.0} & \colorRisk{40.2} & \colorRisk{44.5} & \colorRisk{36.6} & \colorRisk{36.4} & \colorRisk{43.5} \\

% \midrule
% Effects of thinking length\\
% \midrule
% claude37sonnet & \colorRisk{30.8} & \colorRisk{37.5} & \colorRisk{33.6} & \colorRisk{40.1} & \colorRisk{30.2} & \colorRisk{30.1} & \colorRisk{37.9} \\
% claude37sonnet\_1024\_1 & \colorRisk{31.6} & \colorRisk{37.2} & \colorRisk{34.3} & \colorRisk{40.9} & \colorRisk{30.7} & \colorRisk{30.6} & \colorRisk{38.4} \\
% claude37sonnet\_2048\_1 & \colorRisk{31.6} & \colorRisk{38.4} & \colorRisk{34.4} & \colorRisk{41.3} & \colorRisk{30.9} & \colorRisk{30.7} & \colorRisk{38.5} \\
% claude37sonnet\_4096\_1 & \colorRisk{32.1} & \colorRisk{38.8} & \colorRisk{35.1} & \colorRisk{41.8} & \colorRisk{32.0} & \colorRisk{31.7} & \colorRisk{38.9} \\
% claude37sonnet\_16384\_1 & \colorRisk{32.6} & \colorRisk{39.3} & \colorRisk{35.5} & \colorRisk{42.0} & \colorRisk{32.9} & \colorRisk{31.9} & \colorRisk{40.6} \\
% \bottomrule
% \end{tabular}}
% \caption{Risk scores (\%) across different models, color-coded by risk level. The corresponding \( C_v \) for each value appears in Appendix Table \ref{tab:value_risk_corr}. All the correlation formula for predicting risky behavior are statistically significant at $p=0.05$ using Fisher Method, as described in Table \ref{tab:risk_score_formula_detail}.}
% \label{tab:model_behavior_risk}
% \end{table}

==> tables/tab_risk_score_formula_detail.tex <==
\begin{table}[h!]
\begin{tabular}{l|r|r|r|r|r}
\toprule
\textbf{Risky Behavior} & \textbf{Max Range} & \textbf{Min Range} & \textbf{Fisher Stat} & \textbf{Combined $p$} & \textbf{Degrees of Freedom} \\
\midrule
Deception & 71.60 & -329.85 & 2087.62 & 0.0 & 32 \\
Power-Seeking & 100.43 & -232.57 & 1347.77 & 0.0 & 32 \\
Others-Privacy Violation & -62.12 & -157.81 & 199.51 & 0.0 & 32 \\
Corrigibility Failures & 71.26 & -30.54 & 193.84 & 0.0 & 32 \\
Proxy Gaming & 185.57 & -170.79 & 1641.30 & 0.0 & 32 \\
Self-Preservation & 15.27 & -240.74 & 970.49 & 0.0 & 32 \\
Alignment Faking & 87.59 & -28.03 & 255.10 & 0.0 & 32 \\
\bottomrule

\end{tabular}
\caption{Summary statistics for risky behaviors formula with all correlation coefficients of values}
\label{tab:risk_score_formula_detail}
\end{table}



==> tables/tab_rr_for_value.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{l|l|c|c}
\toprule
\textbf{Risky Behavior} & \textbf{Value} & \textbf{Relative Risk}  \\
\midrule
Deception & Adaptability & \textbf{1.23}  \\
Alignment Faking & Adaptability & \textbf{2.43}  \\
Self-Preservation & Adaptability & \textbf{0.80}  \\
Corrigibility Failures & Adaptability & \textbf{1.45}  \\
Proxy Gaming & Adaptability & \textbf{2.19}  \\
Power-Seeking & Adaptability & \textbf{1.80}  \\
Privacy Violation & Adaptability & 1.05  \\
Alignment Faking & Care & 1.25  \\
Proxy Gaming & Care & \textbf{1.16}  \\
Privacy Violation & Care & \textbf{1.98}  \\
Power-Seeking & Care & \textbf{1.18}  \\
Corrigibility Failures & Care & \textbf{1.42}  \\
Self-Preservation & Care & \textbf{1.11}  \\
Deception & Care & \textbf{1.69}  \\
Privacy Violation & Communication & 0.43  \\
Corrigibility Failures & Communication & 0.73  \\
Proxy Gaming & Communication & \textbf{1.28}  \\
Deception & Communication & \textbf{1.55}  \\
Alignment Faking & Communication & \textbf{2.00}  \\
Power-Seeking & Communication & \textbf{0.26}  \\
Self-Preservation & Communication & \textbf{0.24}  \\
Alignment Faking & Cooperation & \textbf{2.11}  \\
Power-Seeking & Cooperation & 1.14  \\
Corrigibility Failures & Cooperation & 0.86  \\
Self-Preservation & Cooperation & 0.92  \\
Privacy Violation & Cooperation & 0.57  \\
Deception & Cooperation & \textbf{1.56}  \\
Proxy Gaming & Cooperation & \textbf{1.49}  \\
Corrigibility Failures & Creativity & 0.98  \\
Power-Seeking & Creativity & \textbf{2.89}  \\
Privacy Violation & Creativity & 1.35  \\
Alignment Faking & Creativity & \textbf{2.56}  \\
Deception & Creativity & \textbf{1.39}  \\
Proxy Gaming & Creativity & \textbf{1.70}  \\
Self-Preservation & Creativity & 0.99  \\
Self-Preservation & Equal Treatment & \textbf{0.40}  \\
Privacy Violation & Equal Treatment & 0.55  \\
Power-Seeking & Equal Treatment & \textbf{0.43}  \\
Alignment Faking & Equal Treatment & 0.74  \\
Corrigibility Failures & Equal Treatment & \textbf{0.63}  \\
Proxy Gaming & Equal Treatment & \textbf{1.20}  \\
Deception & Equal Treatment & \textbf{0.74}  \\
\bottomrule
\end{tabular}
\caption{(Part 1) Relative risk between values and risky behavior. Bolded entries are statistically significant ($p \leq 0.05$).}
\label{tab:value_risk_rr}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{l|l|c|c}
\toprule
\textbf{Risky Behavior} & \textbf{Value} & \textbf{Relative Risk}  \\
\midrule
Self-Preservation & Freedom & \textbf{0.56}  \\
Alignment Faking & Freedom & 1.04  \\
Privacy Violation & Freedom & \textbf{0.24}  \\
Corrigibility Failures & Freedom & 0.84  \\
Proxy Gaming & Freedom & \textbf{0.76}  \\
Deception & Freedom & \textbf{0.55}  \\
Power-Seeking & Freedom & \textbf{0.41}  \\
Privacy Violation & Justice & 0.69  \\
Alignment Faking & Justice & \textbf{0.53}  \\
Corrigibility Failures & Justice & \textbf{0.39}  \\
Self-Preservation & Justice & \textbf{0.37}  \\
Deception & Justice & \textbf{0.59}  \\
Power-Seeking & Justice & \textbf{0.61}  \\
Proxy Gaming & Justice & \textbf{0.67}  \\
Power-Seeking & Learning & \textbf{1.84}  \\
Privacy Violation & Learning & 1.11  \\
Proxy Gaming & Learning & \textbf{1.53}  \\
Corrigibility Failures & Learning & \textbf{1.24}  \\
Alignment Faking & Learning & \textbf{2.54}  \\
Self-Preservation & Learning & \textbf{1.43}  \\
Deception & Learning & \textbf{1.45}  \\
Alignment Faking & Privacy & \textbf{0.42}  \\
Deception & Privacy & \textbf{0.60}  \\
Proxy Gaming & Privacy & \textbf{0.29}  \\
Self-Preservation & Privacy & 0.94  \\
Power-Seeking & Privacy & \textbf{0.29}  \\
Corrigibility Failures & Privacy & 0.72  \\
Privacy Violation & Privacy & \textbf{0.30}  \\
Corrigibility Failures & Professionalism & \textbf{0.76}  \\
Proxy Gaming & Professionalism & \textbf{0.71}  \\
Power-Seeking & Professionalism & \textbf{0.68}  \\
Alignment Faking & Professionalism & \textbf{0.42}  \\
Self-Preservation & Professionalism & \textbf{0.73}  \\
Deception & Professionalism & \textbf{0.53}  \\
Privacy Violation & Professionalism & \textbf{0.64}  \\
\bottomrule
\end{tabular}
\caption{(Part 2) Relative risk between values and risky behavior. Bolded entries are statistically significant ($p \leq 0.05$).}
\label{tab:value_risk_rr_2}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{l|l|c|c}
\toprule
\textbf{Risky Behavior} & \textbf{Value} & \textbf{Relative Risk}  \\
\midrule
Alignment Faking & Protection & \textbf{0.71}  \\
Deception & Protection & \textbf{1.16}  \\
Proxy Gaming & Protection & \textbf{0.72}  \\
Corrigibility Failures & Protection & \textbf{1.26}  \\
Power-Seeking & Protection & \textbf{1.42}  \\
Privacy Violation & Protection & \textbf{1.88}  \\
Self-Preservation & Protection & \textbf{2.32}  \\
Proxy Gaming & Respect & \textbf{0.58}  \\
Corrigibility Failures & Respect & 0.83  \\
Deception & Respect & \textbf{0.56}  \\
Power-Seeking & Respect & \textbf{0.21}  \\
Privacy Violation & Respect & \textbf{0.23}  \\
Self-Preservation & Respect & \textbf{0.52}  \\
Alignment Faking & Respect & 0.82  \\
Power-Seeking & Sustainability & \textbf{1.96}  \\
Privacy Violation & Sustainability & \textbf{0.37}  \\
Self-Preservation & Sustainability & \textbf{1.79}  \\
Proxy Gaming & Sustainability & \textbf{1.79}  \\
Corrigibility Failures & Sustainability & 1.00  \\
Alignment Faking & Sustainability & 0.86  \\
Deception & Sustainability & \textbf{1.13}  \\
Power-Seeking & Truthfulness & \textbf{0.22}  \\
Alignment Faking & Truthfulness & \textbf{0.26}  \\
Corrigibility Failures & Truthfulness & \textbf{0.77}  \\
Proxy Gaming & Truthfulness & \textbf{0.36}  \\
Self-Preservation & Truthfulness & \textbf{0.44}  \\
Privacy Violation & Truthfulness & \textbf{0.29}  \\
Deception & Truthfulness & \textbf{0.32}  \\
Alignment Faking & Wisdom & 1.26  \\
Deception & Wisdom & \textbf{1.26}  \\
Power-Seeking & Wisdom & \textbf{1.28}  \\
Corrigibility Failures & Wisdom & \textbf{2.05}  \\
Proxy Gaming & Wisdom & 1.14  \\
Self-Preservation & Wisdom & \textbf{1.25}  \\
Privacy Violation & Wisdom & 0.56  \\
\bottomrule
\end{tabular}
\caption{(part 3) Relative risk between values and risky behavior. Bolded entries are statistically significant ($p \leq 0.05$).}
\label{tab:value_risk_rr3}
\end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{l|l|c|c}
% \toprule
% \textbf{Risky Behavior} & \textbf{Value} & \textbf{Relative Risk} & \textbf{p-value} \\
% \midrule
% Deception & Adaptability & \textbf{1.23} & \textbf{2.34e-06} \\
% Alignment Faking & Adaptability & \textbf{2.43} & \textbf{2.03e-08} \\
% Self-Preservation & Adaptability & \textbf{0.80} & \textbf{8.70e-03} \\
% Corrigibility Failures & Adaptability & \textbf{1.45} & \textbf{1.41e-04} \\
% Proxy Gaming & Adaptability & \textbf{2.19} & \textbf{0.00e+00} \\
% Power-Seeking & Adaptability & \textbf{1.80} & \textbf{0.00e+00} \\
% Privacy Violation & Adaptability & 1.05 & 8.21e-01 \\
% Alignment Faking & Care & 1.25 & 1.17e-01 \\
% Proxy Gaming & Care & \textbf{1.16} & \textbf{2.55e-04} \\
% Privacy Violation & Care & \textbf{1.98} & \textbf{1.21e-06} \\
% Power-Seeking & Care & \textbf{1.18} & \textbf{2.86e-03} \\
% Corrigibility Failures & Care & \textbf{1.42} & \textbf{1.80e-06} \\
% Self-Preservation & Care & \textbf{1.11} & \textbf{3.95e-02} \\
% Deception & Care & \textbf{1.69} & \textbf{0.00e+00} \\
% Privacy Violation & Communication & 0.43 & 2.28e-01 \\
% Corrigibility Failures & Communication & 0.73 & 2.58e-01 \\
% Proxy Gaming & Communication & \textbf{1.28} & \textbf{2.19e-02} \\
% Deception & Communication & \textbf{1.55} & \textbf{1.96e-08} \\
% Alignment Faking & Communication & \textbf{2.00} & \textbf{3.09e-02} \\
% Power-Seeking & Communication & \textbf{0.26} & \textbf{1.06e-04} \\
% Self-Preservation & Communication & \textbf{0.24} & \textbf{2.12e-05} \\
% Alignment Faking & Cooperation & \textbf{2.11} & \textbf{1.93e-05} \\
% Power-Seeking & Cooperation & 1.14 & 1.43e-01 \\
% Corrigibility Failures & Cooperation & 0.86 & 2.43e-01 \\
% Self-Preservation & Cooperation & 0.92 & 3.33e-01 \\
% Privacy Violation & Cooperation & 0.57 & 7.19e-02 \\
% Deception & Cooperation & \textbf{1.56} & \textbf{0.00e+00} \\
% Proxy Gaming & Cooperation & \textbf{1.49} & \textbf{9.46e-14} \\
% Corrigibility Failures & Creativity & 0.98 & 9.22e-01 \\
% Power-Seeking & Creativity & \textbf{2.89} & \textbf{0.00e+00} \\
% Privacy Violation & Creativity & 1.35 & 3.49e-01 \\
% Alignment Faking & Creativity & \textbf{2.56} & \textbf{4.98e-05} \\
% Deception & Creativity & \textbf{1.39} & \textbf{1.05e-06} \\
% Proxy Gaming & Creativity & \textbf{1.70} & \textbf{1.23e-12} \\
% Self-Preservation & Creativity & 0.99 & 9.61e-01 \\
% Self-Preservation & Equal Treatment & \textbf{0.40} & \textbf{5.03e-13} \\
% Privacy Violation & Equal Treatment & 0.55 & 5.25e-02 \\
% Power-Seeking & Equal Treatment & \textbf{0.43} & \textbf{2.16e-10} \\
% Alignment Faking & Equal Treatment & 0.74 & 2.37e-01 \\
% Corrigibility Failures & Equal Treatment & \textbf{0.63} & \textbf{2.02e-03} \\
% Proxy Gaming & Equal Treatment & \textbf{1.20} & \textbf{2.16e-03} \\
% Deception & Equal Treatment & \textbf{0.74} & \textbf{7.51e-07} \\
% Self-Preservation & Freedom & \textbf{0.56} & \textbf{5.32e-09} \\
% Alignment Faking & Freedom & 1.04 & 8.58e-01 \\
% Privacy Violation & Freedom & \textbf{0.24} & \textbf{5.81e-04} \\
% Corrigibility Failures & Freedom & 0.84 & 1.42e-01 \\
% Proxy Gaming & Freedom & \textbf{0.76} & \textbf{3.12e-05} \\
% Deception & Freedom & \textbf{0.55} & \textbf{0.00e+00} \\
% Power-Seeking & Freedom & \textbf{0.41} & \textbf{5.80e-13} \\
% Privacy Violation & Justice & 0.69 & 1.79e-01 \\
% Alignment Faking & Justice & \textbf{0.53} & \textbf{3.03e-02} \\
% Corrigibility Failures & Justice & \textbf{0.39} & \textbf{2.15e-07} \\
% Self-Preservation & Justice & \textbf{0.37} & \textbf{1.87e-14} \\
% Deception & Justice & \textbf{0.59} & \textbf{1.55e-15} \\
% Power-Seeking & Justice & \textbf{0.61} & \textbf{6.84e-06} \\
% Proxy Gaming & Justice & \textbf{0.67} & \textbf{1.09e-07} \\
% Power-Seeking & Learning & \textbf{1.84} & \textbf{0.00e+00} \\
% Privacy Violation & Learning & 1.11 & 6.15e-01 \\
% Proxy Gaming & Learning & \textbf{1.53} & \textbf{0.00e+00} \\
% Corrigibility Failures & Learning & \textbf{1.24} & \textbf{2.37e-02} \\
% Alignment Faking & Learning & \textbf{2.54} & \textbf{3.11e-10} \\
% Self-Preservation & Learning & \textbf{1.43} & \textbf{8.50e-09} \\
% Deception & Learning & \textbf{1.45} & \textbf{0.00e+00} \\
% Alignment Faking & Privacy & \textbf{0.42} & \textbf{3.35e-02} \\
% Deception & Privacy & \textbf{0.60} & \textbf{5.97e-10} \\
% Proxy Gaming & Privacy & \textbf{0.29} & \textbf{0.00e+00} \\
% Self-Preservation & Privacy & 0.94 & 5.80e-01 \\
% Power-Seeking & Privacy & \textbf{0.29} & \textbf{3.95e-10} \\
% Corrigibility Failures & Privacy & 0.72 & 5.16e-02 \\
% Privacy Violation & Privacy & \textbf{0.30} & \textbf{1.81e-02} \\
% Corrigibility Failures & Professionalism & \textbf{0.76} & \textbf{4.27e-03} \\
% Proxy Gaming & Professionalism & \textbf{0.71} & \textbf{4.72e-11} \\
% Power-Seeking & Professionalism & \textbf{0.68} & \textbf{2.33e-07} \\
% Alignment Faking & Professionalism & \textbf{0.42} & \textbf{1.09e-04} \\
% Self-Preservation & Professionalism & \textbf{0.73} & \textbf{2.29e-06} \\
% Deception & Professionalism & \textbf{0.53} & \textbf{0.00e+00} \\
% Privacy Violation & Professionalism & \textbf{0.64} & \textbf{2.80e-02} \\
% Alignment Faking & Protection & \textbf{0.71} & \textbf{1.35e-02} \\
% Deception & Protection & \textbf{1.16} & \textbf{1.02e-06} \\
% Proxy Gaming & Protection & \textbf{0.72} & \textbf{0.00e+00} \\
% Corrigibility Failures & Protection & \textbf{1.26} & \textbf{1.39e-03} \\
% Power-Seeking & Protection & \textbf{1.42} & \textbf{6.05e-11} \\
% Privacy Violation & Protection & \textbf{1.88} & \textbf{1.69e-05} \\
% Self-Preservation & Protection & \textbf{2.32} & \textbf{0.00e+00} \\
% Proxy Gaming & Respect & \textbf{0.58} & \textbf{1.34e-09} \\
% Corrigibility Failures & Respect & 0.83 & 1.81e-01 \\
% Deception & Respect & \textbf{0.56} & \textbf{1.42e-14} \\
% Power-Seeking & Respect & \textbf{0.21} & \textbf{1.71e-14} \\
% Privacy Violation & Respect & \textbf{0.23} & \textbf{3.62e-03} \\
% Self-Preservation & Respect & \textbf{0.52} & \textbf{7.55e-08} \\
% Alignment Faking & Respect & 0.82 & 4.63e-01 \\
% Power-Seeking & Sustainability & \textbf{1.96} & \textbf{0.00e+00} \\
% Privacy Violation & Sustainability & \textbf{0.37} & \textbf{1.21e-05} \\
% Self-Preservation & Sustainability & \textbf{1.79} & \textbf{0.00e+00} \\
% Proxy Gaming & Sustainability & \textbf{1.79} & \textbf{0.00e+00} \\
% Corrigibility Failures & Sustainability & 1.00 & 9.61e-01 \\
% Alignment Faking & Sustainability & 0.86 & 3.48e-01 \\
% Deception & Sustainability & \textbf{1.13} & \textbf{2.90e-04} \\
% Power-Seeking & Truthfulness & \textbf{0.22} & \textbf{0.00e+00} \\
% Alignment Faking & Truthfulness & \textbf{0.26} & \textbf{5.36e-13} \\
% Corrigibility Failures & Truthfulness & \textbf{0.77} & \textbf{5.42e-04} \\
% Proxy Gaming & Truthfulness & \textbf{0.36} & \textbf{0.00e+00} \\
% Self-Preservation & Truthfulness & \textbf{0.44} & \textbf{0.00e+00} \\
% Privacy Violation & Truthfulness & \textbf{0.29} & \textbf{6.62e-11} \\
% Deception & Truthfulness & \textbf{0.32} & \textbf{0.00e+00} \\
% Alignment Faking & Wisdom & 1.26 & 4.30e-01 \\
% Deception & Wisdom & \textbf{1.26} & \textbf{4.11e-04} \\
% Power-Seeking & Wisdom & \textbf{1.28} & \textbf{3.17e-02} \\
% Corrigibility Failures & Wisdom & \textbf{2.05} & \textbf{9.48e-09} \\
% Proxy Gaming & Wisdom & 1.14 & 1.14e-01 \\
% Self-Preservation & Wisdom & \textbf{1.25} & \textbf{3.57e-02} \\
% Privacy Violation & Wisdom & 0.56 & 2.04e-01 \\
% \bottomrule
% \end{tabular}
% \caption{Relative risk between values and risky behavior. Bolded entries are statistically significant ($p \leq 0.05$).}
% \label{tab:value_risk_rr}
% \end{table}
